$\nu$-LPA: Fast GPU-based Label Propagation Algorithm (LPA) for Community Detection

Community detection is the problem of identifying natural divisions in networks. Efficient parallel algorithms for identifying such divisions are critical in a number of applications. This report presents an optimized implementation of the Label Propagation Algorithm (LPA) for community detection, featuring an asynchronous LPA with a Pick-Less (PL) method every 4 iterations to handle community swaps, ideal for SIMT hardware like GPUs. It also introduces a novel per-vertex hashtable with hybrid quadratic-double probing for collision resolution. On an NVIDIA A100 GPU, our implementation, $\nu$-LPA, outperforms FLPA (sequential), NetworKit LPA (multicore), Gunrock LPA (GPU), and cuGraph Louvain (GPU) by 364x, 62x, 2.6x, and 37x, respectively, while running FLPA and NetworKit LPA on a server with dual 16-core Intel Xeon Gold 6226R processors - processing 3.0B edges/s on a 2.2B edge graph - and achieves 4.7% higher modularity than FLPA, but 6.1% and 9.6% lower than NetworKit LPA and cuGraph Louvain.

==> src/fig-optatomic.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:optatomic--runtime}
    \includegraphics[width=0.98\linewidth]{out/optatomic-runtime.pdf}
  } \\[-2ex]
  \caption{Relative Runtime for hashtable where you check for only empty slot on failed \texttt{atomicCAS()} compared to when you check also for failed \texttt{atomicCAS()} with the desired key as well (in case another thread was attempting to add the same key to the same slot).}
  \label{fig:optatomic}
\end{figure}


==> src/fig-optcoalesced.tex <==
\begin{figure}[hbtp]
  \centering
  \subfigure{
    \label{fig:optcoalesced--runtime}
    \includegraphics[width=0.98\linewidth]{out/optcoalesced-runtime.pdf}
  } \\[-2ex]
  \caption{Relative Runtime for our current approach for hashtable (\textit{Default}), compared to a hashtable based on 
\textit{Coalesced Hashing}.}
  \label{fig:optcoalesced}
\end{figure}


==> src/tab-compare.tex <==
\begin{table}[hbtp]
  \centering
  \caption{Speedup of our multicore implementation of Leiden algorithm compared to other state-of-the-art implementations. Direct comparisons entail running the given implementation on our servers, while indirect comparisons (marked with a $*$, explained in Section \ref{sec:comparison-indirect}) involve comparing results relative to a common reference\ignore{(original Leiden)}.\ignore{Notably, the Leiden implementations vary in their classification, with some being multi-core and others multi-node.}}
  \label{tab:compare}
  \begin{tabular}{|c|c||c|}
    \toprule
    \textbf{Leiden implementation} &
    \textbf{Parallelism} &
    \textbf{Our Speedup} \\
    \midrule
    Original Leiden \cite{com-traag19} & Sequential & $436\times$ \\ \hline
    igraph Leiden \cite{csardi2006igraph} & Sequential & $104\times$ \\ \hline
    NetworKit Leiden \cite{staudt2016networkit} & Parallel & $8.2\times$ \\ \hline
    cuGraph Leiden \cite{kang2023cugraph} & Parallel (GPU) & $3.0\times$ \\ \hline
    ParLeiden-S \cite{huparleiden} & Parallel & $18\times^*$ \\ \hline
    ParLeiden-D (8 nodes) \cite{huparleiden} & Multi-node & $22\times^*$ \\ \hline
  \bottomrule
  \end{tabular}
\end{table}

